Modules and PQ-trees in Robinson spaces

A Robinson space is a dissimilarity space $(X,d)$ on $n$ points for which there exists a compatible order, {\it i.e.} a total order $<$ on $X$ such that $x<y<z$ implies that $d(x,y)\le d(x,z)$ and $d(y,z)\leq d(x,z)$. Recognizing if a dissimilarity space is Robinson has numerous applications in seriation and classification. A PQ-tree is a classical data structure introduced by Booth and Lueker to compactly represent a set of related permutations on a set $X$. In particular, the set of all compatible orders of a Robinson space are encoded by a PQ-tree. An mmodule is a subset $M$ of $X$ which is not distinguishable from the outside of $M$, {\it i.e.} the distances from any point of $X\setminus M$ to all points of $M$ are the same. Mmodules define the mmodule-tree of a dissimilarity space $(X,d)$. Given $p\in X$, a $p$-copoint is a maximal mmodule not containing $p$. The $p$-copoints form a partition of $X\setminus \{p\}$. There exist two algorithms recognizing Robinson spaces in optimal $O(n^2)$ time. One uses PQ-trees and one uses a copoint partition of $(X, d)$. In this paper, we establish correspondences between the PQ-trees and the mmodule-trees of Robinson spaces. More precisely, we show how to construct the mmodule-tree of a Robinson dissimilarity from its PQ-tree and how to construct the PQ-tree from the odule-tree. To establish this translation, additionally to the previous notions, we introduce the notions of $\delta$-graph $G_\delta$ of a Robinson space and of $\delta$-mmodules, the connected components of $G_\delta$. We also use the dendrogram of the subdominant ultrametric of $d$. All these results also lead to optimal $O(n^2)$ time algorithms for constructing the PQ-tree and the mmodule tree of Robinson spaces.

==> sec_8_balls.tex <==
Given two (not necessarily Robinson) dissimilarity spaces $(X,d)$ and $(X,d')$ on the same set $X$, there are three types 
of equivalences  between these two spaces: (i) having the same set of balls, (ii) having the same sets of mmodules, and, in case of Robinson spaces, (iii) having the same PQ-tree, which  is equivalent to (iv) having the same sets of compatible orders. However, as we show below there are no links between the 
equivalences (i), (ii), and (iii), except that (i) implies the conditions (ii) and (iii). 

\begin{proposition}\label{THEOREM_ball_mmodule_PQ_tree}
  Let $(X,d)$ and $(X,d')$ be two dissimilarity spaces on the same set $X$. If $(X,d)$ and $(X,d')$ have the same set of balls, 
  then they have the same set of mmodules and the same mmodule tree. 
  Moreover, if $(X, d)$ is Robinson, then so is $(X, d')$ and  $(X, d)$  and  $(X, d')$ have the same PQ-tree. 
\end{proposition}


\begin{proof}
  Let $M$ be an mmodule of $(X,d)$. Then for any $x\in X\setminus M$, we have
  $M \subset B_{d(x,M)}(x)$. Furthermore,  for any $r<d(x,M)$, we have
  $M\cap B_r(x) = \varnothing$. So
  $M = \bigcap_{x\notin M}{B_{d(x,M)}(x)} \setminus \bigcup_{x\notin M}{B_{d(x,M)-\epsilon}(x)}$. 
  Conversely, let $S$ be a subset of $X$ that  for some values $\delta_x$ can be written as 
  $S = \bigcap_{x\notin S}{B_{\delta_x}(x)} \setminus \bigcup_{x\notin S}{B_{\delta_x-\epsilon}(x)}$.  
  Then $S$ is an mmodule of $(X,d)$ because the distance between $x\notin S$ and every point in $S$ is $\delta_x$. 
  
  Similarly, a set $M'\subset X$ is an mmodule of $(X,d')$ if and only if for some values $\delta_x$, 
  $M' = \bigcap_{x\notin M'}{B'_{\delta_x}(x)} \setminus \bigcup_{x\notin S}{B'_{\delta_x-\epsilon}(x)}$, where $B'_r(x)$ is the 
  ball of radius $r$ centered at $x$ of $(X,d')$.  Since  $(X,d)$ and $(X,d')$ have the same set of balls, 
  they sets of mmodules must coincide. Consequently, $(X,d)$ and $(X,d')$ have the same mmodule tree.

A dissimilarity is Robinson if its ball set form an interval hypergraph; so if $(X, d)$ is Robinson and have the same ball set that $(X, d')$, then $(X, d')$ is a Robinson space.
  Since the PQ-tree of a Robinson dissimilarity is built from its balls,
  if $(X,d)$ and $(X,d')$ have the same ball set, they have the same PQ-tree.
\end{proof}

\Cref{FIGURE_ctre_ex_ball_module,FIGURE_ctre_ex_module_PQ_tree} present
counterexamples to the other potential links. Additionally, $(X,d)$ and $(X,d')$ may 
have the same sets of mmodules, and one be a Robinson space and another a non-Robinson 
space. For this, it suffices in  the dissimilarity space from
\Cref{FIGURE_ctre_ex_module_PQ_tree} to set  $d(t,u) := 10$. Then we
do not modify the mmodules of $(X,d)$, but this new dissimilarity space is not longer 
Robinson. Conversely, we have the following observation: 

\begin{proposition}
  Let $(X, d)$ be a dissimilarity space and $\TM$ be its mmodule tree.
  Then there exists a Robinson space $(X, d_R)$ which has $\TM$ 
  as its mmodule tree.
\end{proposition}

\begin{proof}
  It is possible, in \Cref{algo:mtopq}, not to consider the dissimilarity. We can for instance, at \Cref{line:pq4}   randomly order  the set $X /\M_{\max}$ and skip the lines \ref{line:pq7}--\ref{line:pq14bis}. So we obtain, from every mmodule tree $\TM$ a PQ-tree $\TPQ$.
   Then it is easy to construct, from $\TPQ$, a Robison dissimilarity having
  $\TPQ$ as PQ-tree and $\TM$ as mmodule-tree: we just have to avoid
  making a Q-node conical.
\end{proof}


\begin{center}
  \begin{figure}[h]
    {\scriptsize{
        $$
        \begin{array}{c}
          x\\ y\\z\\ t\\ u \\ v
        \end{array}
        \begin{array}{ccccccc}
          0 & 1 & 2 & 3 & 3 & 6 \\
            & 0 & 1 & 3 & 3 & 5 \\
            & & 0 & 3 & 3 & 4 \\
            & & & 0 & 1 & 3\\
            & & & & 0 & 3 \\
            & &  & &  & 0
        \end{array}
        \hspace{2cm}
        \begin{array}{c}
          x\\ y\\z\\ t\\ u \\ v
        \end{array}
        \begin{array}{ccccccc}
          0 & 1 & 5 & 3 & 3 & 6 \\
            & 0 & 4 & 3 & 3 & 5 \\
            & & 0 & 3 & 3 & 1 \\
            & & & 0 & 1 & 3\\
            & & & & 0 & 3 \\
            & &  & &  & 0
        \end{array}
        \hspace{.6cm}
        \begin{array}{c}
          x\\ y\\t\\ u\\ z \\ v
        \end{array}
        \begin{array}{ccccccc}
          0 & 1 & 3 & 3 & 5 & 6 \\
            & 0 & 3 & 3 & 4 & 5 \\
            & & 0 & 1 & 3 & 3 \\
            & & & 0 & 1 & 3\\
            & & & & 0 & 3 \\
            & &  & &  & 0
        \end{array}
        $$
      }}
    \begin{tikzpicture}[scale=.4]
      \begin{scope}[xshift=1.7cm]
        \draw(0,0) -- (6,0) -- (6,.7) -- (0,.7) -- (0,0) ;
        \draw(.5,0)-- (.5,-1) node[below]{\footnotesize{$x$}} ;
        \draw(1.5,0)-- (1.5,-.95) node[below]{\footnotesize{$y$}} ;
        \draw(2.5,0)-- (2.5,-1) node[below]{\footnotesize{$z$}} ;
        \draw(4,0) -- (4,-.4) ;
        \draw(4, -.6) circle(.2) ;
        \draw(3.84, -.7) -- (3.5, -1) node[below]{\footnotesize{$t$}} ;
        \draw(4.16, -.7) -- (4.5, -1) node[below]{\footnotesize{$u$}} ;
        \draw(5.5,0)-- (5.5,-1) node[below]{\footnotesize{$v$}} ;
      \end{scope}

      \begin{scope}[xshift = 21cm]
        \draw(0,0) -- (6,0) -- (6,.7) -- (0,.7) -- (0,0) ;
        \draw(.5,0)-- (.5,-1) node[below]{\footnotesize{$x$}} ;
        \draw(1.5,0)-- (1.5,-.95) node[below]{\footnotesize{$y$}} ;
        \draw(4.5,0)-- (4.5,-1) node[below]{\footnotesize{$z$}} ;
        \draw(3,0) -- (3,-.4) ;
        \draw(3, -.6) circle(.2) ;
        \draw(2.84, -.7) -- (2.5, -1) node[below]{\footnotesize{$t$}} ;
        \draw(3.16, -.7) -- (3.5, -1) node[below]{\footnotesize{$u$}} ;
        \draw(5.5,0)-- (5.5,-1) node[below]{\footnotesize{$v$}} ;
      \end{scope}
      \begin{scope}[xshift = 31cm]
        \draw(0,0) node{$\,$};
      \end{scope}
    \end{tikzpicture}
    \caption{\small{Two dissimilarities having the same mmodules (in
        both cases, the trivial mmodules and $\{x,y,z,v \}$) but not
        the same PQ-tree.}}
    \label{FIGURE_ctre_ex_module_PQ_tree}
  \end{figure}
\end{center}


\begin{center}
  \begin{figure}[h]
    {\scriptsize{
        $$
        \begin{array}{c}
          x\\ y\\z\\ t\\ u
        \end{array}
        \begin{array}{cccccc}
          0 & 1 & 2 & 3 & 4 \\
            & 0 & 1 & 1 & 1 \\
            & & 0 & 1 & 1 \\
            & & & 0 & 1 \\
            & & & & 0
        \end{array}
        \hspace{.6cm}
        \begin{array}{c}
          x\\ y\\z\\ t\\ u
        \end{array}
        \begin{array}{ccccc}
          0 & 1 & 2 & 3 & 4 \\
            & 0 & 1 & 1 & 3 \\
            & & 0 & 1 & 2 \\
            & & & 0 & 1 \\
            & & & & 0 \\
        \end{array}
        \hspace{1.5cm}
        \begin{array}{c}
          x\\ y\\z\
        \end{array}
        \begin{array}{ccc}
          0 & 1 & 2 \\
            & 0 & 1 \\
            & & 0 \\
        \end{array}
        \hspace{.6cm}
        \begin{array}{c}
          x\\ y\\z
        \end{array}
        \begin{array}{ccc}
          0 & 1 & 3 \\
            & 0 & 2 \\
            & & 0 \\
        \end{array}
        $$
      }}
    \caption{\small{{\sc Left}: Two dissimilarities having the same
        mmodules (only the trivial ones) and the same PQ-tree (a
        Q-node with children, in this order, $x,y,z,t,u$) but not the
        same balls: except the singletons, the balls are $\{x,y\}$,
        $\{x,y,z\}$, $\{x,y,z,t\}$, $\{x,y,z,t,u\}$, $\{y,z,t,u\}$ for
        the dissimilarity on the left and $\{x,y\}$, $\{x,y,z\}$,
        $\{x,y,z,t\}$, $\{x,y,z,t,u\}$, $\{t,u\}$, $\{z,t,u\}$,
        $\{y,z,t,u\}$, \{y,z,t\} for the dissimilarity on the right.
        {\sc Right}: Two dissimilarities having the same PQ-tree (a
        Q-node with children, in this order, $x, y, z$) but not the
        same mmodules: the dissimilarity on the right has no
        non-trivial mmodules, but $\{x,z\}$ is an mmodule of the
        dissimilarity on the left.} }
    \label{FIGURE_ctre_ex_ball_module}
  \end{figure}
\end{center}



